Algebraic and Combinatorial Tools for State Complexity : Application to the Star-Xor Problem

We investigate the state complexity of the star of symmetrical differences using modifiers and monsters. A monster is an automaton in which every function from states to states is represented by at least one letter. A modifier is a set of functions allowing one to transform a set of automata into one automaton. These recent theoretical concepts allow one to find easily the desired state complexity. We then exhibit a witness with a constant size alphabet.

==> eptcsdata.tex <==
\providecommand{\firstpage}{154}
\providecommand{\publicationstatus}{J. Leroux and J.-F. Raskin (Eds.): Tenth International Symposium\\ on Games, Automata, Logics, and Formal Verification (GandALF'19).\\
EPTCS 305, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.305.11}{10.4204/EPTCS.305.11}}
\pdfoutput=1

